Growth of Stationary Hastings-Levitov

We construct and study a stationary version of the Hastings-Levitov$(0)$ model. We prove that, unlike in the classical HL$(0)$ model, in the stationary case the size of particles attaching to the aggregate is tight, and therefore SHL$(0)$ is proposed as a potential candidate for a stationary off-lattice variant of Diffusion Limited Aggregation (DLA). The stationary setting, together with a geometric interpretation of the harmonic measure, yields new geometric results such as stabilization, finiteness of arms and arm size distribution. We show that, under appropriate scaling, arms in SHL$(0)$ converge to the graph of Brownian motion which has fractal dimension $3/2$. Moreover we show that trees with $n$ particles reach a height of order $n^{2/3}$, corresponding to a numerical prediction of Meakin from 1983 for the gyration radius of DLA growing on a long line segment.

==> scaling_limits.tex <==
% !TEX root = HL_welldeff.tex
% ********************************************************************************************************************************
\section{Typical height and particle size}
\label{sec:scaling}
%
%A natural variation on the SHL(0) model is to attach slit particles of length $\delta$, corresponding to slit map $\tilde{s}^\delta(z)=\sqrt{z^2 - \delta^2}$, at positions of the rescaled Poisson process $\delta P$ and then analyse the corresponding conformal mappings in the limit as $\delta \to 0$. Due to scale invariance of the half-plane, this is equivalent to analysing the original model with slit particles of length 1, under the rescaling
%\[
%F^{\delta}_{t}(z) = \delta F_{\delta^{-1} t}(\delta^{-1}z)
%\]  
%as $\delta \to 0$.
%
%Before analysing the rescaled process, we begin with a preliminary lemma on the standard backward process. 
 
\begin{lemma}\label{lem:prelimto_all_powerful}
Suppose $\tilde \mu$ is a backward $\mathrm{SHL}(0)$ process. Then
\[
\ev \left [ \tilde F_t(z) \right ]= z+i \pi t/2
\]
and
\[
\ev \left [ \tilde F'_t(z) \right ]= 1.
\]

Furthermore, There exists some absolute constant $C>0$ such that, for each $z \in \HH$ and $t \in [0,\infty)$, 
\begin{equation}\label{eq:concval}
\ev \left [ \sup_{s \leq t} \left | \tilde F_s(z) - (z+i \pi s/2) \right |^2\right ] \leq \frac{C t}{1+\Im z},
\end{equation}
and
\begin{equation}\label{eq:concder}
\ev \left [ \sup_{s \leq t} \left | \tilde F'_s(z) - 1 \right |^2\right ] \leq \frac{C (1+|\log (\Im z)|) t}{1+(\Im z)^3} \exp \left ( \frac{C (1+|\log (\Im z)|) t}{1+(\Im z)^3} \right ) < \infty,
\end{equation}
where expectation is with respect to $\tilde \mu$.

%\note{These results (in particular the last one) are very weak. There ought to be a way to exploit the fact that $\Im(\tilde F_t(z))$ grows linearly with $t$ but I haven't been able to make it work.}

\end{lemma}
\begin{proof}
Fix $z \in \HH$. Then, using Lemma \ref{lemma:slit_estimates},
\begin{align*}
\tilde F_t(z) 
&= z+ M_t(z) + \lim_{n \to \infty} \int_{0}^t \int_{-n}^n  \left[ \tilde{s}_x(\tilde F_{s}(z)) - \tilde F_{s}(z) \right] dx ds \\
&= z + M_t(z) + i\pi t/2  
\end{align*}
where $\left ( M_t(z) \right )$ is a zero-mean martingale with
\begin{align*}
\ev \left [ |M_t(z)|^2 \right ] 
&= \ev \left [ \int_0^t \int_{-\infty}^\infty \left| \tilde{s}_x(\tilde F_{s}(z)) - \tilde F_{s}(z) \right|^2 dx ds \right ] \\
&\leq \ev \left [ \int_0^t \frac{C}{1+\Im \tilde F_{s}(z)} ds \right ] \\
&\leq \frac{C t}{1+\Im z}.
\end{align*}
Here $C$ is the absolute constant from Lemma \ref{lemma:slit_estimates}. The result follows by Doob's inequality.

Similarly
\[
\tilde F'_t(z) = 1+M'_t(z)
\]
where $\ev \left [ M'_t(z) \right ]=0$ and
\begin{align*}
\ev \left [ |M'_t(z)|^2 \right ] 
&= \ev \left [ \int_0^t |\tilde F'_s(z)|^2 \int_{-\infty}^\infty \left| \tilde{s}'_x(\tilde F_{s}(z)) - 1 \right|^2 dx ds \right ] \\
&\leq \ev \left [ \int_0^t \frac{C |\tilde F'_s(z)|^2(1+|\log (\Im \tilde F_{s}(z))|1_{(\Im \tilde F_{s}(z) < 1)})}{1+(\Im \tilde F_{s}(z))^3} ds \right ] \\
&\leq \frac{2C (1+|\log (\Im z)|) t}{1+(\Im z)^3} + \frac{2C (1+|\log (\Im z)|)}{1+(\Im z)^3} \int_0^t \ev \left [ \sup_{r \leq s} \left | \tilde F'_r(z) - 1 \right |^2\right ] ds.
\end{align*}
The result follows by Doob's inequality and Gronwall's Lemma.
\end{proof}
\begin{corollary}\label{cor:condbound}
Let $Z$ be independent of $\tilde{F}_1(z)$ satisfying $\Im Z>h>0$, then $$\ev[|\tilde{F}_1'(Z)|]\le 1+\frac{C\log h}{1+h^3}.$$
\end{corollary}\label{cor:function_lln}
The second corollary that we will need is a law of large numbers behavior for $\Im \tilde{F}_t(0)$. Abbreviate the event $\mathfs{G}_T=\{\forall t>T, \Im \tilde{F}_t(0)>t/2\}.$
\begin{corollary}
 For every $\epsilon>0$ there is a $t_0>0$ such that $\prob(\mathfs{G}_{t_0})>1-\epsilon$.
\end{corollary}

\begin{proof} Let $t_n=n^2$. By Lemma \ref{lem:prelimto_all_powerful},
\begin{align}
\prob\left(\Im \tilde{F}_{t_n}(0)<\frac{t_n}{1.9}\right)\le \prob\left(\left|\tilde{F}_{t_n}(0)-\frac{i\pi t_n}{2}\right|^2>\frac{t_n^2}{4}\right)<\frac{C}{t_n}=\frac{C}{n^2}.
\end{align}
By Borel-Cantelli with probability $1$ there is some $N\in\BN$ such that for all $n>N$, $\Im \tilde{F}_{t_n}(0)>\frac{t_n}{1.9}$. Now for every $(n-1)^2<t<n^2$ with $n>N$, using the monotonicity in time of the imaginary part of the process we obtain
$$
\Im \tilde{F}_t(0)\ge\Im \tilde{F}_{(n-1)^2}(0) >\frac{(n-1)^2}{1.9}=\frac{n^2}{1.9}\frac{(n-1)^2}{n^2}>\frac{t}{2}
,$$
where the last inequality holds for large enough $n$. Finally the Lemma follows since $\lim_{t\rightarrow\infty}\prob(\mathfs{G}_t)=\prob(\exists t_0\forall t>t_0~\Im \tilde{F}_t(0)>t/2)=1$.
\end{proof}

Next we prove tightness for the particles size. 
We start with Theorem \ref{thm:derbndproc} which governs the derivative of the mapping on the boundary.
\begin{theorem}\label{thm:derbndproc}
For every $\epsilon>0$ there is a $M>0$ such that for all $t>0$ $$\prob\left(|\tilde{F}'_t(0)|>M\right)<\epsilon.$$
\end{theorem}
\begin{proof}
Let $\epsilon>0$. By Corollary \ref{cor:function_lln} there is a $t_0>0$ such that $\prob(\mathfs{G}_{t_0})>1-\epsilon$.
Define a sequence of i.i.d functions $\{G_i(z)\}_{i\ge1}$ distributed like $\tilde{F}_1(z)$. Then by the Markov property (Lemma \ref{prop:markov}) the following equalities holds in distribution $\forall n>t_0$,
\begin{equation}
\tilde{F}_n(z)=G_n\circ G_{n-1}\circ\cdots\circ G_{1}(z) =G_n\circ G_{n-1}\circ\cdots\circ G_{t_0+1}\circ\tilde{F}_{t_0}(z) .
\end{equation}
Using the chain rule we can write:
\bae
\tilde{F}'_n(0)=&G_n'(G_{n-1}\circ G_{n-2}\circ\cdots\circ G_1(0))\cdot G_{n-1}'(G_{n-2}\circ\cdots\circ G_1(0))\cdots\\
\cdot &G_{n-2}'(G_{n-3}\circ\cdots\circ G_1(0))\cdots G_{t_0+1}'(\tilde{F}_{t_0}(0))\cdot\tilde{F}_{t_0}'(0)
\eae
Now if we condition on the event $\mathfs{G}_{t_0}$ by Corollary \ref{cor:condbound} we get
\begin{equation}
\ev\left[|G_n'(G_{n-1}\circ G_{n-2}\circ\cdots\circ G_1(0))|\cdots |{G}_{t_0+1}'(\tilde{F}_{t_0}(0))|\bigg|\mathfs{G}_{t_0}\right]\le\prod_{m=t_0}^n\left(1+\frac{C\log m}{m^3}\right),
\end{equation}
which converges to $1$ as $t_0\rightarrow\infty$ and $n\ge t_0$.
The last estimate we use which is the reason we only prove tightness and not present moment bounds is that for every $t_0,\epsilon>0$ there is a $\tilde{M}$ such that $\prob(|\tilde{F}'_{t_0}(0)|>\tilde{M})<\epsilon$. This follows from the fact that the process is well defined. Now abreviate $\tilde{\mathfs{G}}_{t_0}={\mathfs{G}}_{t_0}\cap\{\tilde{F}'_{t_0}(0)|<\tilde{M}\}$.
Since
\bae
\prob(|\tilde{F}_n'(0)|<M)\ge\prob(|\tilde{F}_n'(0)|<M|\tilde{\mathfs{G}}_{t_0})\prob(\tilde{\mathfs{G}}_{t_0})
\eae
we can given $\epsilon$ choose and $M,\tilde{M}>0$ and $t_0\in\BN$ such that both elements in the RHS are larger than $(1-\epsilon)$ yielding $\prob(|\tilde{F}_n'(0)|>M)<2\epsilon$.

\end{proof}

\newcommand{\particle}{{\bf P}}
\newcommand{\diam}{\mathrm{diam}}



We now continue to implement Theorem \ref{thm:derbndproc} in order to control the actual size of the particle. Fix $t>0$ and
let $\hat P$ be the Poisson process $P$ with an extra point at $(t,0)$. Let $\hat F$ be the SHL process driven by $\hat P$. We define the particle arriving at time $t$ as the difference between the ranges of $\hat F_t$ and $\hat F_{t-}$, and denote it by $\particle_t$
\begin{theorem}\label{thm:prtszbnd} 
For every $\epsilon>0$ there exists $M$ such that for every $t$,
\[
P[\diam(\particle_t) > M] < \epsilon.
\]
\end{theorem}

%\ref{eq:concval} \ref{eq:concder}

\begin{proof}
Note that $\particle_t = \hat F_{t-} \big((0,i]\big)$ and therefore 
\[
\diam(\particle_t) \leq \int_0^1 |\hat{F}_{t-}'(ix)|dx\le \sup_{0\le x\le 1}|\hat{F}_{t-}'(ix)|
\]
Now from the well definability of the process we have that $\forall t_0>0,\forall\epsilon>0,\exists M>0$ such that $\prob(\sup_{0\le x\le 1}|\hat{F}_{t_0}'(ix)|>M)<\epsilon$. By the continuity of the process on $\mathbb{R}\cup\BH$ we have that for every $\epsilon>0$ there is an $\eta>0$ small enough such that $$\prob\left(\forall t>t_0, \inf_{0\le s\le \eta}\Im \hat{F}_t(is)>t/2\Big|\mathfs{G}_{t_0}\right)>1-\epsilon.$$
$$
$$

The tightness of the integral $\int_0^\eta |\hat{F}_{t-}'(ix)|dx$ follows from Theorem \ref{thm:derbndproc}. For the rest of the interval, we can repeat $1/\eta$ times the same distortion theorem argument explained in the proof of Theorem \ref{thm:constworks}. We get that
$$
\sup_{\eta\le s\le 1}||\hat{F}_{t-}'(is)|\le 16^{1/\eta}|\hat{F}_{t-}'(i\eta)|
.$$
Proving the tightness of $\diam(\particle_t)$.
\end{proof}


%We now wish to estimate the average height of the process and the size of a particle attached in the average height. Since we are working in the stationary case the average height of a point in which a particle attaches is given by the half-plane capacity. 
%\begin{definition}
%Let $B_t$ be complex Brownian motion, and define $\tau=\inf\{t>0:B_t\in \tilde{F}_t(\partial\BH)\}$. Define the half-plane capacity 
%$$
%{\rm hcap}(\tilde{F}_t(\partial\BH))=\lim_{y\rightarrow\infty}\ev^{iy}[\ima(B_\tau)]
%.$$
%\end{definition}
%By the proof of Lemma \ref{lem:prelimto_all_powerful} Since $F_t(z) = z + M_t(z) + i\pi t/2$ and $M_t(z)$ is zero mean martingale which decays to $0$ as $z\rightarrow\infty$ we obtain
%\begin{corollary}
%$$
%{\rm hcap}(\tilde{F}_t(\partial\BH))=\pi t/2
%.$$
%\end{corollary}
%
%We can now state the main result about particle sizes, mainly the average size of a particle attaching at a typical height is bounded.
%\begin{corollary}
%There is a constant $c>0$ such that for all $t>0$
%$$
%\ev\left[|\tilde{F}_t'(i\cdot{\rm hcap}(\tilde{F}_t(\partial\BH)))\right]\le c
%.$$
%\end{corollary}
%\begin{proof}
%Follows by the bound in Lemma \ref{lem:prelimto_all_powerful} evaluated at $z=i\pi t/2$.
%\end{proof}
%The following corollary is an immediate consequence of this lemma, via the scaling relationship and the connection between the forward and backwards SHL processes.
%
%\begin{corollary}\label{lem:all_powerful}
%Suppose $\mu$ is a $\mathrm{SHL}(0)$ process. Then
%\[
%\ev \left [ F_t(z) \right ]= z+i \pi t/2 = \ev \left [ F^\delta_t(z) \right ]
%\]
%and
%\[
%\ev \left [ F'_t(z) \right ]= 1 = \ev \left [ (F^\delta_t)'(z) \right ].
%\]
%Furthermore
%\[
%F^{\delta}_{t}(z) \to z + it
%\]
%in probability as $\delta \to 0$.
%\end{corollary}
%
%Suppose that $(t,x) \in \delta P$. By the standard arc-length formula, the length of the particle added at position $x$ at time $t$ is given by
%\[
%\delta_{(t,x)}= \int_0^\delta |(F^\delta)'_{t-}(x+iu)|du.
%\]
%The following result tells us that particle sizes are of approximately constant size in the rescaled SHL(0) model when the particle sizes are small.
% 
%\begin{theorem}
%As $\delta \to 0$,
%\[
%\ev \left [ \left . \left |\delta^{-1}\delta_{(t,x)} - 1 \right |^2 \right | (t,x) \in \delta P \right ] \to 0.
%\]
%\end{theorem}
%\begin{proof}
%By definition
%\[
%\delta^{-1}\delta_{(t,x)}= \int_0^1 |F'_{(\delta^{-1} t)-}(\delta^{-1}x+iu)|du
%\]
%and hence, by Cauchy-Schwarz,
%\[
%\ev \left [ \left . \left |\delta^{-1}\delta_{(t,x)} - 1 \right |^2 \right | (t,x) \in \delta P \right ]
%\leq \int_0^1 \ev \left [ \left |F'_{(\delta^{-1} t)-}(\delta^{-1}x+iu)- 1\right |^2 \right ] du.
%\]
%\note{I would like to use dominated convergence here to finish off the proof, but the exponential blow-up when $u$ is close to zero is problematic. Any ideas?}
%
%\end{proof}

